Rethinking Likelihood distributions: Student's t Likelihood Boosts Bayesian Neural Network Performance

In Bayesian neural networks (BNNs), variational inference is a widely adopted framework for modeling uncertainty in a distributional way, with the evidence lower bound (ELBO) serving as the standard objective function. Several distributions contribute to the ELBO loss, such as the prior, approximated posterior, and likelihood distribution. Typically, these distributions are all approximated by a Gaussian distribution, since it is easy to compute, allows for reparameterized gradients, and provides a closed-form loss for training. However, several works have highlighted that this assumption may not generally hold, posing the risk of model misspecification. Alternative distributions have been proposed for the prior specifically, while the effect of distribution choice on the likelihood distribution remains unexplored. In this work, our aim is to close this gap by investigating whether alternative assumptions for the likelihood distribution can outperform the commonly used Gaussian. We compare several likelihood distribution assumptions, such as skewed or heavy-tailed, across regression tasks on both artificial and real-world datasets using standard multilayer perceptrons (MLPs). Our findings demonstrate that Student's t yields better predictive performance than a Gaussian likelihood distribution, independent of the data distribution and MLP architecture (depth and width). In some cases, Student's t can also lead to shorter training times, while still being easy to implement.

==> tables/table2.tex <==
\begin{table}[!h]
\caption{Significance table for the generalization to more noise types with noise scale (std) 3. We included four more noise types (Cauchy, Laplace, lognormal, and Uniform) in this experiment. Rows are grouped by noise type (Gaussian, Gamma, Student’s $t$, Cauchy, Laplace, lognormal, and Uniform). For each model architecture ($\text{depth}\times \text{width}$) and sample size $n\in\{300, 3{,}000, 30{,}000\}$, the table reports--separately for MSE and CRPS (lower is better)--which assumed predictive distribution attains the best test score. An asterisk indicates the significance of an unpaired t-test comparing the marked choice against each of the other two. For results with error distribution Gaussian, Gamma, and Student's $t$, see \Cref{tab:table_exp1}\\}\label{tab:table_exp2}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llllllll}
\hline
    && \multicolumn{2}{c}{$n=300$} & \multicolumn{2}{c}{$n=3{,}000$} & \multicolumn{2}{c}{$n=30{,}000$}\\
    \cline{3-8}
    \rule{0pt}{12pt}
    NOISE& MODEL&&&&&&\\
    TYPE & SHAPE & MSE $\downarrow$ & CRPS $\downarrow$& MSE $\downarrow$& CRPS $\downarrow$& MSE $\downarrow$& CRPS $\downarrow$\\
    \hline
    \\[-6pt]
    Cauchy 
    & 1$\times$ 32 & X & G$^{**}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$\\
    & 2$\times$ 16 & T$^{***}$ & X & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$\\
    & 4$\times$ 8 & T$^{***}$ & $\times$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$\\
    & 8$\times$ 4 & X & G$^{*}$ & X & T$^{***}$ & T$^{***}$ & T$^{***}$\\
    \hline
    Laplace 
    & 1$\times$ 32 & X & G$^{***}$ & T$^{***}$ & T$^{**}$ & T$^{***}$ & X\\
    & 2$\times$ 16 & T$^{***}$ & X & T$^{**}$ & T$^{**}$ & T$^{**}$ & X\\
    & 4$\times$ 8 & T$^*$ & X & T$^{***}$ & T$^{***}$ & T$^{***}$ & X \\
    & 8$\times$ 4 & X & X & X & T$^{***}$ & T$^{***}$ & T$^{***}$\\
    \hline
    Log- 
    & 1$\times$ 32 & T$^*$ & G$^*$ & T$^{*}$ & T$^{***}$ & T$^{***}$ & T$^{***}$\\
    normal& 2$\times$ 16 & T$^{***}$ & X & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$\\
    & 4$\times$ 8 & X & $\times$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    & 8$\times$ 4 & X & X & T$^{*}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    \hline
    Uniform 
    & 1$\times$ 32 & X & X & X & T$^{*}$ & X & X\\
    & 2$\times$ 16 & T$^{*}$ & X & T$^{***}$ & X & X & X\\
    & 4$\times$ 8 & X & X & T$^{***}$ & T$^{***}$ & X & X \\
    & 8$\times$ 4 & X & X & T$^{*}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
\hline
\\[-6pt]
\multicolumn{8}{l}{
G: Gaussian\ \
S: skew normal\ \
T: Student's $t$\
}\\
\multicolumn{8}{l}{
X: no significant difference between results of the three predictive distributions.
}\\
\multicolumn{8}{l}{
$^{*}$: $p < 0.05$\ \
$^{**}$: $p < 0.01$\ \
$^{***}$: $p < 0.001$.
}
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/table3.tex <==
\begin{table}[!h]
\caption{Significance table for the generalization to more noise types with noise scale (std) 9. Rows are grouped by noise type (Gaussian, Gamma, Student’s $t$, Cauchy, Laplace, lognormal, and Uniform). For each model architecture ($\text{depth}\times \text{width}$) and sample size $n\in\{300, 3{,}000, 30{,}000\}$, the table reports--separately for MSE and CRPS (lower is better)--which assumed predictive distribution attains the best test score. An asterisk indicates the significance of an unpaired t-test comparing the marked choice against each of the other two.\\}\label{tab:table_exp3}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llllllll}
\hline
    && \multicolumn{2}{c}{$n=300$} & \multicolumn{2}{c}{$n=3000$} & \multicolumn{2}{c}{$n=30000$}\\
    \cline{3-8}
    \rule{0pt}{12pt}
    NOISE& MODEL&&&&&&\\
    TYPE & SHAPE & MSE $\downarrow$& CRPS $\downarrow$& MSE $\downarrow$& CRPS $\downarrow$& MSE $\downarrow$& CRPS $\downarrow$\\
    \hline
    \\[-6pt]
    Gamma 
    & 1$\times$32 & X & G$^{***}$ & T$^{***}$ & T$^{***}$ & X & X \\
    & 2$\times$16 & T$^{***}$ & X & T$^{***}$ & T$^{***}$ & G$^{**}$ & X \\
    & 4$\times$8  & T$^{*}$ & G$^{**}$ & T$^{***}$ & T$^{***}$ & X & X \\
    & 8$\times$4  & X & G$^{*}$ & X & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    \hline
    Gaussian 
    & 1$\times$32 & T$^{***}$ & G$^{*}$ & T$^{*}$ & T$^{*}$ & X & X \\
    & 2$\times$16 & T$^{***}$ & X & T$^{*}$ & T$^{**}$ & X & X \\
    & 4$\times$8  & T$^{***}$ & X & T$^{***}$ & T$^{***}$ & X & X \\
    & 8$\times$4  & X & X & X & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    \hline
    Student T 
    & 1$\times$32 & X & G$^{**}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    & 2$\times$16 & X & G$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & X \\
    & 4$\times$8  & T$^{***}$ & G$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & X \\
    & 8$\times$4  & X & X & T$^{*}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    \hline
    Laplace 
    & 1$\times$32 & X & G$^{**}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & X \\
    & 2$\times$16 & T$^{***}$ & G$^{**}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & X \\
    & 4$\times$8  & T$^{***}$ & G$^{**}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & X \\
    & 8$\times$4  & T$^{**}$ & X & X & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    \hline
    Log- 
    & 1$\times$32 & X & G$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{*}$ & T$^{***}$ \\
    normal& 2$\times$16 & X & G$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & X \\
    & 4$\times$8  & X & G$^{*}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & X \\
    & 8$\times$4  & X & G$^{***}$ & X & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    \hline
    Cauchy 
    & 1$\times$32 & X & G$^{**}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    & 2$\times$16 & X & G$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    & 4$\times$8  & X & G$^{**}$ & X & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    & 8$\times$4  & G$^{*}$ & G$^{***}$ & X & T$^{***}$ & T$^{**}$ & T$^{***}$ \\
    \hline
    Uniform 
    & 1$\times$32 & X & G$^{***}$ & T$^{*}$ & X & G$^{**}$ & X \\
    & 2$\times$16 & T$^{***}$ & G$^{***}$ & T$^{***}$ & X & X & X \\
    & 4$\times$8  & X & G$^{***}$ & T$^{***}$ & T$^{***}$ & X & X \\
    & 8$\times$4  & T$^{*}$ & X & T$^{**}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
\hline
\\[-6pt]
\multicolumn{8}{l}{
G: Gaussian\ \
S: skew normal\ \
T: Student's $t$\
}\\
\multicolumn{8}{l}{
x: no significant difference between results of the three predictive distributions.
}\\
\multicolumn{8}{l}{
$^{*}$: $p < 0.05$\ \
$^{**}$: $p < 0.01$\ \
$^{***}$: $p < 0.001$.
}
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/table4.tex <==
\begin{table}[!h]
\caption{Significance table for the generalization to more noise types with noise scale (std) 15. Rows are grouped by noise type (Gaussian, Gamma, Student’s $t$, Cauchy, Laplace, lognormal, and Uniform). For each model architecture ($\text{depth}\times \text{width}$) and sample size $n\in\{300, 3{,}000, 30{,}000\}$, the table reports--separately for MSE and CRPS (lower is better)--which assumed predictive distribution attains the best test score. An asterisk indicates the significance of an unpaired t-test comparing the marked choice against each of the other two.\\}\label{tab:table_exp4}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llllllll}
\hline
    && \multicolumn{2}{c}{$n=300$} & \multicolumn{2}{c}{$n=3000$} & \multicolumn{2}{c}{$n=30000$}\\
    \cline{3-8}
    \rule{0pt}{12pt}
    NOISE& MODEL&&&&&&\\
    TYPE & SHAPE & MSE $\downarrow$& CRPS $\downarrow$& MSE $\downarrow$& CRPS $\downarrow$& MSE $\downarrow$& CRPS $\downarrow$\\
    \hline
    \\[-6pt]
    Gamma 
    & 1$\times$32 & X & G$^{***}$ & T$^{***}$ & T$^{***}$ & G$^{***}$ & X \\
    & 2$\times$16 & T$^{***}$ & G$^{***}$ & T$^{***}$ & T$^{***}$ & G$^{***}$ & T$^{***}$ \\
    & 4$\times$8  & T$^{*}$ & G$^{**}$ & T$^{***}$ & T$^{***}$ & G$^{***}$ & X \\
    & 8$\times$4  & X & G$^{***}$ & X & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    \hline
    Gaussian 
    & 1$\times$32 & X & G$^{***}$ & T$^{***}$ & T$^{***}$ & X & X \\
    & 2$\times$16 & T$^{***}$ & G$^{***}$ & T$^{***}$ & T$^{***}$ & X & X \\
    & 4$\times$8  & X & T$^{***}$ & T$^{***}$ & G$^{***}$ & X & X \\
    & 8$\times$4  & X & T$^{**}$ & X & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    \hline        
    Student T 
    & 1$\times$32 & X & G$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    & 2$\times$16 & T$^{***}$ & G$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    & 4$\times$8  & T$^{**}$ & G$^{*}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    & 8$\times$4  & X & G$^{**}$ & X & T$^{***}$ & T$^{*}$ & T$^{***}$ \\
    \hline
    Laplace 
    & 1$\times$32 & X & G$^{*}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    & 2$\times$16 & T$^{***}$ & G$^{***}$ & T$^{***}$ & T$^{***}$ & X & X \\
    & 4$\times$8  & X & X & T$^{***}$ & T$^{***}$ & X & X \\
    & 8$\times$4  & X & G$^{*}$ & X & T$^{***}$ & T$^{**}$ & T$^{***}$ \\
    \hline
    Log- 
    & 1$\times$32 & X & G$^{***}$ & T$^{***}$ & T$^{***}$ & X & T$^{***}$ \\
    normal& 2$\times$16 & T$^{*}$ & G$^{**}$ & T$^{***}$ & T$^{***}$ & X & T$^{***}$ \\
    & 4$\times$8  & X & G$^{*}$ & T$^{***}$ & T$^{***}$ & X & T$^{***}$ \\
    & 8$\times$4  & X & X & X & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
    \hline
    Cauchy 
    & 1$\times$32 & G$^{**}$ & G$^{**}$ & T$^{***}$ & T$^{***}$ & T$^{**}$ & T$^{***}$ \\
    & 2$\times$16 & X & X & T$^{*}$ & T$^{**}$ & T$^{***}$ & T$^{***}$ \\
    & 4$\times$8  & G$^{*}$ & G$^{**}$ & T$^{*}$ & T$^{***}$ & T$^{*}$ & T$^{***}$ \\
    & 8$\times$4  & X & X & X & T$^{***}$ & T$^{*}$ & T$^{***}$ \\
    \hline
    Uniform 
    & 1$\times$32 & X & G$^{*}$ & T$^{**}$ & X & G$^{**}$ & X \\
    & 2$\times$16 & T$^{***}$ & G$^{***}$ & T$^{**}$ & X & G$^{***}$ & G$^{***}$ \\
    & 4$\times$8  & X & G$^{***}$ & T$^{***}$ & T$^{***}$ & X & X \\
    & 8$\times$4  & X & X & X & T$^{***}$ & T$^{***}$ & T$^{***}$ \\
\hline
\\[-6pt]
\multicolumn{8}{l}{
G: Gaussian\ \
S: skew normal\ \
T: Student's $t$\
}\\
\multicolumn{8}{l}{
X: no significant difference between the results of the three predictive distributions.
}\\
\multicolumn{8}{l}{
$^{*}$: $p < 0.05$\ \
$^{**}$: $p < 0.01$\ \
$^{***}$: $p < 0.001$.
}
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/table6.tex <==
\begin{table}[!h]
\caption{Significance table for ENTSO-E dataset. For each model architecture ($\text{depth}\times \text{width}$), the table reports--separately for MAE, MAPE, MSE, CRPS, epoch and training time used (lower is better)---which assumed predictive distribution attains the best test score. An asterisk indicates the significance of an unpaired t-test comparing the marked choice against each of the other two.\\}\label{tab:table_real2}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llllllll}
\hline
\rule{0pt}{12pt}
    Dataset & MODEL SHAPE & MAE $\downarrow$& MAPE $\downarrow$& MSE $\downarrow$& CRPS $\downarrow$& EPOCH $\downarrow$& TIME $\downarrow$\\
    \hline
    \\[-6pt]
    ENTSO-E&1$\times$ 4 & T$^{***}$ & T$^{***}$ & T$^{***}$ &T$^{***}$& $\times$ & X \\
    &1$\times$ 16 & T$^{***}$ & T$^{***}$ & T$^{***}$ &T$^{***}$& $\times$ & X \\
    &1$\times$ 32 & T$^{***}$ & T$^{***}$ & T$^{***}$ &T$^{***}$& T$^{***}$ & X \\
    \cline{2-8}
    &4$\times$ 4 & T$^{***}$ & T$^{***}$ & G$^{***}$ &T$^{***}$& T$^{***}$ & T$^{*}$ \\
    &4$\times$ 16 & T$^{***}$ & T$^{***}$ & X &T$^{*}$& X & X \\
    &4$\times$ 32 & T$^{***}$ & T$^{***}$ & T$^{***}$ &T$^{**}$& T$^{***}$ & T$^{***}$ \\
    \cline{2-8}
    &8$\times$ 4 & T$^{***}$ & T$^{***}$ & G$^{***}$ &X& T$^{**}$ & X \\
    &8$\times$ 16 & T$^{***}$ & T$^{***}$ & T$^{***}$ &T$^{***}$& X & X \\
    &8$\times$ 32 & T$^{***}$ & T$^{***}$ & X &T$^{**}$& T$^{***}$ & X \\
\hline
\\[-6pt]
\multicolumn{7}{l}{
G: Gaussian\ \
S: skew normal\ \
T: Student's $t$\
}\\
\multicolumn{7}{l}{
X: no significant difference between the results of the three predictive distributions.
}\\
\multicolumn{7}{l}{
$^{*}$: $p < 0.05$\ \
$^{**}$: $p < 0.01$\ \
$^{***}$: $p < 0.001$.
}
\end{tabular}
\end{adjustbox}
\end{table}
